Bottom-Up 2D Pose Estimation via Dual Anatomical Centers for Small-Scale Persons

In multi-person 2D pose estimation, the bottom-up methods simultaneously predict poses for all persons, and unlike the top-down methods, do not rely on human detection. However, the SOTA bottom-up methods' accuracy is still inferior compared to the existing top-down methods. This is due to the predicted human poses being regressed based on the inconsistent human bounding box center and the lack of human-scale normalization, leading to the predicted human poses being inaccurate and small-scale persons being missed. To push the envelope of the bottom-up pose estimation, we firstly propose multi-scale training to enhance the network to handle scale variation with single-scale testing, particularly for small-scale persons. Secondly, we introduce dual anatomical centers (i.e., head and body), where we can predict the human poses more accurately and reliably, especially for small-scale persons. Moreover, existing bottom-up methods use multi-scale testing to boost the accuracy of pose estimation at the price of multiple additional forward passes, which weakens the efficiency of bottom-up methods, the core strength compared to top-down methods. By contrast, our multi-scale training enables the model to predict high-quality poses in a single forward pass (i.e., single-scale testing). Our method achieves 38.4\% improvement on bounding box precision and 39.1\% improvement on bounding box recall over the state of the art (SOTA) on the challenging small-scale persons subset of COCO. For the human pose AP evaluation, we achieve a new SOTA (71.0 AP) on the COCO test-dev set with the single-scale testing. We also achieve the top performance (40.3 AP) on OCHuman dataset in cross-dataset evaluation.

==> figure_tex/bbox_recall_improvements.tex <==
\pgfplotsset{width=6.2cm,height=4.1cm,compat=1.9}

\begin{figure*}[t]
\centering
\begin{tikzpicture}
\scriptsize
\begin{axis}[
    title={BBR percentage increase on COCO},
    xlabel={Scale of person},
    ylabel={\% increase over SOTA},
    xmin=64, xmax=128,
    ymin=-1, ymax=40,
    xtick={64, 96, 128},
    ytick={-1,10,20,30,40},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (64, 39.1)(96,3.4)(128,-0.9)
    };
    \legend{Our increases}

\addplot[
    color=blue,
    mark=,
    ]
    coordinates {
    (64,14.3)(96,14.3)(128,14.3)
    };
    \addlegendentry{Our avg. increase}
\end{axis}
\end{tikzpicture}
\hskip 10pt
\begin{tikzpicture}
\scriptsize
\begin{axis}[
    title={BBR percentage increase on CrowdPose},
    xlabel={Scale of person},
    ylabel={\% increase over SOTA},
    xmin=64, xmax=128,
    ymin=0, ymax=51,
    xtick={64, 96, 128},
    ytick={0,10,20,30,40,50},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (64, 50.3)(96,18.7)(128,4.5)
    };
    \legend{Our increases}
\addplot[
    color=blue,
    mark=,
    ]
    coordinates {
    (64,16.4)(96,16.4)(128,16.4)
    };
    \addlegendentry{Our avg. increase}
\end{axis}
\end{tikzpicture}
\vspace{-1.0em}
\caption{
The percentage increases of our method over the SOTA methods in BBR evaluation on both COCO and CrowdPose datasets. The best-performed existing methods in all scales (CGNet on COCO and SWAHR on CrowdPose from Table~\ref{tab:bbox_recall_all}) are used as the baseline for percentage improvement calculation at different scales on COCO vadidation set (left) and CrowdPose test set (right).
% \edit{Our percentage}{Percentage} increases of BBR \edit{}{of our method} over the SOTA methods \edit{to the second best model}{} (CGNet for COCO and SWAHR for CrowdPose \edit{}{where the second best BBRs in all scales are achieved respectively}) at different scales on COCO vadidation set (left) and CrowdPose test set (right).
}
\vspace{-1.0em}
\label{fig:bbox_improvments}
\end{figure*}
